Partitioned solution strategies for coupled BEM-FEM acoustic fluid-structure interaction problems

This paper investigates two FEM-BEM coupling formulations for acoustic fluid-structure interaction (FSI) problems, using the Finite Element Method (FEM) to model the structure and the Boundary Element Method (BEM) to represent a linear acoustic fluid. The coupling methods described interconnect fluid and structure using classical or localized Lagrange multipliers, allowing the connection of non-matching interfaces. First coupling technique is the well known mortar method, that uses classical multipliers and is compared with a new formulation of the method of localized Lagrange multipliers (LLM) for FSI applications with non-matching interfaces. The proposed non-overlapping domain decomposition technique uses a classical non-symmetrical acoustic BEM formulation for the fluid, although a symmetric Galerkin BEM formulation could be used as well. A comparison between the localized methodology and the mortar method in highly non conforming interface meshes is presented. Furthermore, the methodology proposes an iterative preconditioned and projected bi-conjugate gradient solver which presents very good scalability properties in the solution of this kind of problems.

==> LaTeXex.tex <==

 
 
%    Equation display glue, modifies PLAIN's -- CAF 
 
\abovedisplayskip 12pt plus 3pt minus 6pt 
\belowdisplayskip 10pt plus 3pt minus 6pt 
\abovedisplayshortskip 0pt plus 3pt 
\belowdisplayshortskip 7pt plus 3pt minus 4pt 
  
%    "Overfull box" tolerance, resets PLAIN's 
 
\hfuzz=15pt \tolerance=500 
 
%    LMSC extensions to PLAIN.TEX for Tex82 -- C. A. Felippa, 9/83 
 

\def \tinyskin  {\par\vskip1pt plus1pt minus1pt\noindent} 
\def \smallskin {\par\smallskip\noindent} 
\def \medskin   {\par\medskip\noindent} 
\def \bigskin   {\par\bigskip\noindent} 
\def \ven {\vfill\eject} 
\def \spr{\noalign{\vskip2pt}}
\def \tinyspr{\noalign{\vskip1pt}}
\def \sprneg{\noalign{\vskip-2pt}}
\def \tinyskip{\vskip 1pt plus .5pt}
\def \b{\bigskip} \def \m{\medskip} \def \s{\smallskip} \def \t{\tinyskip}
\def \sneg{\vskip-\smallskipamount}
\def \mneg{\vskip-\medskipamount}
\def \bneg{\vskip-\bigskipamount}
\def \tneg{\vskip -1pt  plus .5pt minus.5pt}
\def \d{\displaystyle} \def\n{\noindent} \def \t{\textstyle}
\def \return{\hfill\break}

\def \lft#1{#1\hfil}        % leftify argument 
\def \ctr#1{\hfil#1\hfil}   % centerify argument 
\def \rt#1{\hfil#1}         % rightify argument 
 
\def\hangitem#1#2{\setbox9=\hbox to #1{#2\hss}\par\noindent 
                  \hangindent1\wd9\box9}
\def\hangfifteen#1{\setbox9=\hbox to 15pt{#1\hss}\par\noindent 
\hangindent1\wd9\box9} 
\def\hangtwenty#1{\setbox9=\hbox to 20pt{#1\hss}\par\noindent 
\hangindent1\wd9\box9} 
\def\hangthirty#1{\setbox9=\hbox to 30pt{#1\hss}\par\noindent 
\hangindent1\wd9\box9} 
\def\hangforty#1{\setbox9=\hbox to 40pt{#1\hss}\par\noindent 
\hangindent1\wd9\box9} 
\def\hangfifty#1{\setbox9=\hbox to 50pt{#1\hss}\par\noindent 
\hangindent1\wd9\box9} 
\def\hangsixty#1{\setbox9=\hbox to 60pt{#1\hss}\par\noindent 
\hangindent1\wd9\box9} 
\def\hangseventy#1{\setbox9=\hbox to 70pt{#1\hss}\par\noindent 
\hangindent1\wd9\box9} 
\def\hangeighty#1{\setbox9=\hbox to 80pt{#1\hss}\par\noindent 
\hangindent1\wd9\box9} 
\def\hanghundred#1{\setbox9=\hbox to 100pt{#1\hss}\par\noindent 
\hangindent1\wd9\box9} 
\def\hanghundredtwenty#1{\setbox9=\hbox to 120pt{#1\hss}\par\noindent 
\hangindent1\wd9\box9} 
\def\hanghundredforty#1{\setbox9=\hbox to 140pt{#1\hss}\par\noindent 
\hangindent1\wd9\box9} 
\def\hanghundredsixty#1{\setbox9=\hbox to 160pt{#1\hss}\par\noindent 
\hangindent1\wd9\box9} 
\def\itemitemitem{\par\indent\indent 
                   \hangindent3\parindent \textindent} 
\def\itemitemitemitem{\par\indent\indent\indent 
                   \hangindent4\parindent \textindent} 
 
%         Boxing text  (Note: \boxed in in mathex.tex)
 
\long\def\boxtwohundred#1{\setbox0=\vbox{\hsize 200pt 
    \noindent{#1}} \hbox{\lower.8pt\hbox{\lower 
 10pt\hbox{\lower 1\dp0\hbox{\vbox{\hrule height .8pt \hbox{\vrule 
 width .8pt \hskip 10pt\vbox{\vskip 10pt\box0\vskip10pt}\hskip 10pt 
 \vrule width .8pt}\hrule height .8pt}}}}}} 
\long\def\boxtwohundredfifty#1{\setbox0=\vbox{\hsize 250pt 
    \noindent{#1}} \hbox{\lower.8pt\hbox{\lower 
 12.5pt\hbox{\lower 1\dp0\hbox{\vbox{\hrule height .8pt \hbox{\vrule 
 width .8pt \hskip12.5pt\vbox{\vskip 12.5pt\box0\vskip 12.5pt}\hskip 12.5pt 
 \vrule width .8pt}\hrule height .8pt}}}}}} 
\long\def\boxthreehundred#1{\setbox0=\vbox{\hsize 300pt 
    \noindent{#1}} \hbox{\lower.8pt\hbox{\lower 
 12.5pt\hbox{\lower 1\dp0\hbox{\vbox{\hrule height .8pt \hbox{\vrule 
 width .8pt \hskip 12.5pt\vbox{\vskip 12.5pt\box0\vskip 12.5pt}\hskip 12.5pt 
 \vrule width .8pt}\hrule height .8pt}}}}}} 
\long\def\boxthreehundredfifty#1{\setbox0=\vbox{\hsize 350pt 
    \noindent{#1}} \hbox{\lower.8pt\hbox{\lower 
 12.5pt\hbox{\lower 1\dp0\hbox{\vbox{\hrule height .8pt \hbox{\vrule 
 width .8pt \hskip 12.5pt\vbox{\vskip 12.5pt\box0\vskip 12.5pt}\hskip 12.5pt 
 \vrule width .8pt}\hrule height .8pt}}}}}} 
 \long\def\boxthreehundredeighty#1{\setbox0=\vbox{\hsize 380pt 
    \noindent{#1}} \hbox{\lower.8pt\hbox{\lower 
 12.5pt\hbox{\lower 1\dp0\hbox{\vbox{\hrule height .8pt \hbox{\vrule 
 width .8pt \hskip 12.5pt\vbox{\vskip 12.5pt\box0\vskip 12.5pt}\hskip 12.5pt 
 \vrule width .8pt}\hrule height .8pt}}}}}}
 
\def\boxedtext#1{\boxed{\vbox{\halign{\ctr{##}\cr#1\cr}}}}
\def\phantomboxedtext#1{\vbox{\halign{\ctr{##}\cr#1\cr}}}
\def\boxedtextwidth#1.#2{\boxed{\vbox{\halign to#1{\ctr{##}\cr#2\cr}}}}
\def\boxedparagraph#1.#2{\boxed{\vbox{\halign{\quad\vtop{
    \parindent=0pt\hsize=#1 \strut##\strut}\quad\cr#2\cr}}}}


%        Preps for environment definitions
 

\def\plainbaselines{
                    \lineskip\plainlineskip
                    \baselineskip\plainbaselineskip 
                    \lineskiplimit\plainlineskiplimit
                    }
\def\plaindisplayskip{
                      \abovedisplayskip=12pt plus 3pt minus 9pt
                      \abovedisplayshortskip=0pt plus 3pt
                      \belowdisplayskip=12pt plus 3pt minus 9pt
                      \belowdisplayshortskip=7pt plus 3pt minus 4pt
                     } 

 

%\input mathex           % Math extensions 
%\input verbatim         % verbatim macros 



